Distributed Online Learning via Cooperative Contextual Bandits

In this paper we propose a novel framework for decentralized, online learning by many learners. At each moment of time, an instance characterized by a certain context may arrive to each learner; based on the context, the learner can select one of its own actions (which gives a reward and provides information) or request assistance from another learner. In the latter case, the requester pays a cost and receives the reward but the provider learns the information. In our framework, learners are modeled as cooperative contextual bandits. Each learner seeks to maximize the expected reward from its arrivals, which involves trading off the reward received from its own actions, the information learned from its own actions, the reward received from the actions requested of others and the cost paid for these actions - taking into account what it has learned about the value of assistance from each other learner. We develop distributed online learning algorithms and provide analytic bounds to compare the efficiency of these with algorithms with the complete knowledge (oracle) benchmark (in which the expected reward of every action in every context is known by every learner). Our estimates show that regret - the loss incurred by the algorithm - is sublinear in time. Our theoretical framework can be used in many practical applications including Big Data mining, event detection in surveillance sensor networks and distributed online recommendation systems.

==> cascaded.tex <==
\section{Online Learning in Cascaded Classifier Systems}

Different from the previous sections, in this section I assume that the classifiers are cascaded. The goal is to make a correct classification in a delay sensitive environment. When an input data stream arrives, it is forwarded to one of ${\cal M}$ classifiers. The classifier has three options. It can label the data as {\em classified} and return the label, label it as {\em irrelevant} and discard it, or label it as {\em further investigation is needed} and send it to another classifier. 

The goal is to learn which classification order is optimal for each arriving data $x(t)$. Note that there are $M!$ classification orders for each data, therefore even the optimization problem is very difficult to solve. However, it can be solved easily in an online setting. The learning algorithm choses an order $\sigma(1), \sigma(2), \ldots, \sigma(M)$ at each time step. For instance assume that for data input $x$, $\sigma(1), \sigma(2)$ is an optimal order. After a {\em classified} decision by the second classifier in the chain, the server not only updates the reward of the classification order $\sigma(1), \sigma(2), \ldots, \sigma(M)$, but it can update the rewards of all classification orders starting with $\sigma(1), \sigma(2)$. If you think of each arm as a classification order, then this learning problem exploits the correlation between the arms. I also propose to use a zooming type algorithm here. By this we don't have to worry about how the data arrives. 

We can also explore more complex classifier structures such as chains of classifiers working in parallel with different input data streams, but they can call each other sometimes to benefit from experience of other classifiers. 

==> centralized.tex <==
\section{An Optimal Classification Scheme with Perfect Information} \label{sec:centralized}

Our benchmark when evaluating the performance of the learning algorithms is the optimal distributed solution which is computed offline given the complete knowledge about the data arrival process and classifier accuracies. 
%For simplicity, we focus on the distributed classification problem of classifier $i$ 
In the optimal classification scheme, for each context $x \in {\cal X}$ classifier $i$ wants to find the optimal classification function from the set $\cup_{i \in {\cal M}} {\cal F}_i$, i.e., the classification function $k$ with the highest accuracy minus the cost of classification $d_k$. We assume that the context space and classification accuracies have the following structural property:
%
\begin{assumption} \label{ass:lipschitz}
For each $k \in \cup_{i \in {\cal M}} {\cal F}_i$, there exists $L>0$, $\alpha>0$ such that for all $x,x' \in {\cal X}$
%
\begin{align*}
|\pi_k(x) - \pi_k(x')| \leq L |x-x'|^\alpha.
\end{align*}
%
\end{assumption}
%
Assumption \ref{ass:lipschitz} indicates that the accuracy of a classifier for similar contexts will be similar to each other. For example, when the context is the time of the day, population density which affects the classifier accuracy at times $x$ and $x'$ will be close to each other when the times $x$ and $x'$ are close to each other. Therefore the relation between classifier accuracy and time can be written down as a Lipschitz condition.  


\rev{For a set $A$ let $|A|$ denote the cardinality of that set.} In this section, we assume that the optimal classification scheme for any classifier $i$ 
partitions ${\cal X}$ into  $|\cup_{i \in {\cal M}} {\cal F}_i|$ sets in each of which a single classification function is optimal.
%Note that partitioning $[-1,1]^d$ is not enough because the noise can carry a data point outside of $[-1,1]^d$.
In order to solve this problem exactly, classifier $i$ needs to know the classification function that yields the \rev{lowest expected cost} for each $x \in {\cal X}$, which is computationally intractable. Assume for an instance that everything is known. Classifier $i$ has access to all classification functions $\cup_{i \in {\cal M}} {\cal F}_i$ and it knows $q_i$. Then the optimal solution for classifier $i$ is given by the following optimization problem.  
%
\begin{problem}\label{prob:opt}
When the classifier accuracies for each context $x \in {\cal X}$ is completely known, the optimal classification regions
%
\begin{align*}
{\cal R}^* = \{R^*_k\}_{(k \in \cup_{i \in {\cal M}} {\cal F}_i)},
\end{align*}
%
of ${\cal X}$ are the solution of 
%
\begin{align}
\textrm{{\bf (P1)  }} {\cal R}^* = \argmin_{{\cal R} \in \Theta} E \left[ \left| Y - \sum_{k \in \cup_{i \in {\cal M}} {\cal F}_i} k(X) I(X \in R_l) \right| + \sum_{k \in {\cal F}_i} d_k I(X \in R_k) + \sum_{k \in {\cal M}_{-i}}  d_k I \left(X \in \cup_{j \in {\cal F}_k} R_j \right)   \right], \label{eqn:opt}
\end{align}
%
where $\Theta$ is the set of $|\cup_{i \in {\cal M}} {\cal F}_i|$-set partitions of ${\cal X}$, the expectation is taken with respect to the distribution $q_i$ and $Y$ is the random variable denoting the true label. Here $I(X \in R_l)$ denotes the event that data received by the classifier belongs to the $l$th set of the partition ${\cal R}$ of ${\cal X}$.
%
\end{problem}

Note that ${\cal R}^*$ depends on $d_k$. Although, we made no assumptions on $d_k$s, in general exchanging data and label with other classifiers is more costly for a classifier then using its own classification function. Therefore without loss of generality we can assume that $d_l > d_k$ for $l \in {\cal M}_{-i}$, $k \in {\cal F}_i$.
%
The complexity of finding the optimal classification regions increases exponentially with $|\cup_{i \in {\cal M}} {\cal F}_i|$. The learning problem we are trying to solve is even harder because the classifiers are distributed, so each classifier cannot directly access to all classifier functions (classifier $i$ only knows set ${\cal F}_i$ and ${\cal M}$, but it does not know any ${\cal F}_j, j \in {\cal M}_{-i}$), and the distributions $q_i$, $i \in {\cal M}$ are unknown. Therefore, we need to use online learning techniques that does not rely on solving the optimization problem in given (\ref{eqn:opt}) or an estimated version of it. 

==> numerical.tex <==
%\vspace{-0.05in}
\section{Numerical Results} \label{sec:numerical}

In this section we provide numerical results for our proposed algorithms CoS and DCZA using network security data from KDD Cup 1999 data set. We compare the performance of our learning algorithms with {\em AdaBoost} \cite{freund1995desicion} and the online version of AdaBoost called {\em sliding window AdaBoost} \cite{oza2001online}. 

The network security data has 42 features. The goal is to predict at any given time if an attack occurs or not based on the values of the features.
%
We run the simulations for three different context information; (i) context is the label at the previous time step, (ii) context is the feature named {\em srcbytes}, which is the number of data bytes from source to destination, (iii) context is time. All the context information is normalized to be in $[0,1]$. There are $4$ local learners. Each local learner has $2$ classification functions. Classification costs $d_k$ is set to $0$ for all $k \in {\cal K}_1$.

%Difference from Luca's data: classifier 3 is all one, classifier 8 is all zero
All classification functions are trained using 5000 consecutive samples from different segments of the network security data. Then, they are tested on $T = 20000$ consecutive samples. We run simulations for two different sets of classifiers. 
%
In our first simulation S1, there are two good classifiers that have low number of errors on the test data, while in our second simulation S2, there are no good classifiers. The types of classification functions used in S1 and S2 are given in Table \ref{tab:sim_setup} along with the number of errors each of these classification functions made on the test data. From Table \ref{tab:sim_setup} we can observe that the error percentage of the best classification function is $3$ in S1, while it is $47$ in S2. A situation like in S2 can appear when the distribution of the data changes abruptly so that the classification functions trained on the old data becomes inaccurate for the new data. In our numerical results we will show how the context information can be used to improve the performance in both S1 and S2.
%
The accuracies of the classifiers on the test data are unknown to the learners so they cannot simply choose the best classification function. 
%
In all our simulations, we assume that the test data sequentially arrives to the system and the label is revealed to the algorithms with a one step delay. 

\begin{table}[t]
\centering
{\fontsize{8}{6}\selectfont
\setlength{\tabcolsep}{.1em}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Learner & 1 &2 &3 & 4\\
\hline
Classification  & Naive Bayes,  &Always $1$, & RBF Network, & Random Tree,  \\
Function (S1)  & Logistic & Voted Perceptron &J48 & Always $0$\\
\hline
 Error  & 47,  & 53,  & 47, & 47,  \\
percentage (S1) & 3 & 4 &  47 & 47\\
\hline
 Classification  & Naive Bayes,  &Always $1$,  & RBF Network,  & Random Tree,  \\
Function (S2) & Random & Random & J48 & Always $0$ \\
\hline
 Error & 47,  & 53,  & 47,  & 47,  \\ 
percentage (S2) & 50 & 50 & 47 & 47 \\
\hline
\end{tabular}
}
\add{\vspace{-0.1in}}
\caption{Simulation setup}
\vspace{-0.25in}
\label{tab:sim_setup}
\end{table}

Since we only consider single dimensional context, $d=1$. However, due to the bursty, non-stochastic nature of the network security data we cannot find a value $\alpha$ for which Assumption \ref{ass:lipschitz2} is true. Nevertheless, we consider two cases, C1 and C2, given in Table \ref{tab:par_setup}, for CoS and DCZA parameter values.
%
In C2, the parameters for CoS and DCZA are selected according to Theorems \ref{theorem:cos} and \ref{thm:adaptivemain}, assuming $\alpha=1$. 
%
In C1, the parameter values are selected in a way that will limit exploration and training. However, the regret bounds in Theorems \ref{theorem:cos} and \ref{thm:adaptivemain} may not hold for these values. 

\begin{table}[t]
\centering
{\fontsize{8}{6}\selectfont
\setlength{\tabcolsep}{.3em}
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
 & $D_1(t)$ & $D_2(t)$ & $D_3(t)$ & $m_T$ & $A$ & $p$ \\
\hline
(C1) CoS & $t^{1/8} \log t$ & $2 t^{1/8} \log t$ & $t^{1/8} \log t$ & $\lceil T \rceil^{1/4}$ & & \\
\hline
(C1) DCZA & $t^{1/8} \log t$ & $2 t^{1/8} \log t$ & $t^{1/8} \log t$ &  & $1$ & $4$ \\
\hline
(C2) CoS & $t^{1/2} \log t$ & $2 t^{1/2} \log t$ & $t^{1/2} \log t$ & $\lceil T \rceil^{1/4}$ & & \\
\hline
(C2) DCZA & $t^{2/p} \log t$ & $2 t^{2/p} \log t$ & $t^{2/p} \log t$ &  & $1$ & $(3+\sqrt{17})/2$ \\
\hline
\end{tabular}
}
\add{\vspace{-0.05in}}
\caption{Parameters for CoS and DCZA}
\label{tab:par_setup}
\add{\vspace{-0.4in}}
\end{table}

In our simulations we consider the performance of learner 1. Table \ref{tab:sim_results} shows under each simulation and parameter setup the percentage of errors made by CoS and DCZA and the percentage of time steps spent in training and exploration phases for learner 1. We compare the performance of DCZA and CoS with AdaBoost and sliding window AdaBoost (SWA) whose error rates are also given in Table \ref{tab:sim_results}. AdaBoost and SWA are trained using 20000 consecutive samples from the data set different from the test data. 
%
SWA re-trains itself in an online way using the last $w$ observations, which is called the window length. Both AdaBoost and SWA are ensemble learning methods which require learner 1 to combine the predictions of all the classification functions. Therefore, when implementing these algorithms we assume that learner 1 has access to all classification functions and their predictions, whereas when using our algorithms we assume that learner 1 only has access to its own classification functions and other learners but not their classification functions. Moreover, learner 1 is limited to use a single prediction in CoS and DCZA. This may be the case in a real system when the computational capability of local learners are limited and the communication costs are high.

First, we consider the case when the parameter values are as given in C1. We observe that when the context is the previous label, CoS and DCZA perform better than AdaBoost and SWA for both S1 and S2. This result shows that although CoS and DCZA only use the prediction of a single classification function, by exploiting the context information they can perform better than ensemble learning approaches which combine the predictions of all classification functions. We see that the error percentage is smallest for CoS and DCZA when the context is the previous label.
% 
This is due to the bursty nature of the attacks.
%
The exploration percentage for the case when context is the previous label is larger for DCZA than CoS. 
As we discussed in Section \ref{sec:reduction}, the number of explorations of DCZA can be reduced by utilizing the observations from the old hypercube to learn about the accuracy of the arms in a newly activated hypercube. When the context is the feature of the data or the time, for S1, CoS and DCZA perform better than AdaBoost while SWA with window length $w=100$ can be slightly better than CoS and DCZA. But again, this difference is not due to the fact that CoS and DCZA makes too many errors. It is because of the fact that CoS and DCZA explores and trains other classification functions and learners. AdaBoost and SWA does not require these phases. But they require communication predictions of all classification functions and communication of all local learners with each other at each time step. Moreover, SWA re-trains itself by using the predictions and labels in its time window, which makes it computationally inefficient.
%
Another observation is that using the feature as context is not very efficient when there are no good classifiers (S2). However, the error percentages of CoS and DCZA ($39\%$ and $38\%$ respectively) are still lower than the error percentage of the best classifier in S2 which is $47\%$.
\comment{
In Figure \ref{fig:CoS_res} and \ref{fig:DCZA_res}, the number of classification errors is given as a function of time for CoS and DCZA, respectively for S1 and C1, for all three different context information. The error function is {\em spike-shaped} because of the training phases that happens when a change in the context occurs. Note that when the context is previous label or {\em srcbytes}, the spikes follow the changes in the data, while when the context is time, the spikes are uniformly distributed. 

\begin{figure}
\begin{center}
\includegraphics[width=0.8\columnwidth]{CoS_res}
\caption{Number of errors made by CoS as a function of time.} 
\label{fig:CoS_res}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=0.8\columnwidth]{DCZA_res}
\caption{Number of errors made by DCZA as a function of time.} 
\label{fig:DCZA_res}
\end{center}
\end{figure}
}

We observe that both CoS and DCZA performs poorly when the set of parameters is given by C2.
This is due to the fact that the percentage of training and exploration phases is too large for C2, thus these algorithms cannot exploit the information they gathered efficiently. Another important reason for the poor performance is the short time horizon. As the time horizon grows, we expect the exploration and training rates to decrease, and the exploitation rate to increase which will improve the performance. 



\begin{table}[t]
\centering
{\fontsize{8}{6}\selectfont
\setlength{\tabcolsep}{.3em}
\begin{tabular}{|l|c|c|c|}
\hline
(S1, S2) & Error $\%$ & Training $\%$ & Exploration $\%$  \\
\hline
(C1,S1) CoS & 0.7, 4.6, 4.8 & 0.3, 3, 2.8 & 1.4, 6.3, 8.5 \\
\hline
(C1,S1) DCZA & 1.4, 3.5, 3.2 & 0.4, 1.3, 0.9 & 4, 5.9, 7 \\
\hline
(C1,S2) CoS & 0.9, 39, 10 & 0.3, 3, 2.8 & 1.5, 6.5, 8.6 \\
\hline
(C1,S2) DCZA & 1.9, 38, 4.8 & 0.4, 1.3, 1 & 4, 6, 7 \\
\hline
(C2,S1) CoS & 16, 14, 41 & 8.5, 16, 79 & 55 27 20\\
\hline
(C2,S1) DCZA & 31, 29, 29 & 33 19 87 & 66 66 12 \\
\hline
(S1, S2) AdaBoost & 4.8, 53 & & \\
\hline
(S1, S2) SWA ($w=100$) & 2.4, 2.7 & &\\
\hline
(S2, S2) SWA ($w=1000$) & 11, 11 & & \\
\hline
\end{tabular}
}
\add{\vspace{-0.05in}}
\caption{Simulation Results}
\label{tab:sim_results}
\vspace{-0.4in}
\end{table}













